Joint and individual analysis of breast cancer histologic images and genomic covariates

A key challenge in modern data analysis is understanding connections between complex and differing modalities of data. For example, two of the main approaches to the study of breast cancer are histopathology (analyzing visual characteristics of tumors) and genetics. While histopathology is the gold standard for diagnostics and there have been many recent breakthroughs in genetics, there is little overlap between these two fields. We aim to bridge this gap by developing methods based on Angle-based Joint and Individual Variation Explained (AJIVE) to directly explore similarities and differences between these two modalities. Our approach exploits Convolutional Neural Networks (CNNs) as a powerful, automatic method for image feature extraction to address some of the challenges presented by statistical analysis of histopathology image data. CNNs raise issues of interpretability that we address by developing novel methods to explore visual modes of variation captured by statistical algorithms (e.g. PCA or AJIVE) applied to CNN features. Our results provide many interpretable connections and contrasts between histopathology and genetics.

==> sections/dep/old_intro_next_try.tex <==
Histopathology is the classical approach to diagnosing and studying cancer, dating back to the 1800s \citep{rosen2001rosen, titford2006short}.
 First, a tissue sample is taken from a patient, processed and chemically stained with \textit{Hematoxylin and Eosin} (Figure \ref{fig:he_example}).
The stained tissue is then visually examined by a pathologist under a microscope who makes various determinations such as: nuclear grade, histologic subtype, etc.
Increasingly,  genetic information is also used to understand the biological processes underlying cancer as well as predict patient prognosis and response to treatments \citep{gyHorffy2015multigene}. 

Typically pathology and genetics are pursued independently.
For example, genetic test results may arrive weeks after a clinician has reviewed the pathology report.
While some attempts have been made to merge these two approaches, these have mostly been qualitative \todo{melissa cite something here?}.
There is now a demand -- both by researchers and clinicians -- for quantitative integration approaches \cite{ash2018joint, couture2018image, chen2019pathomic}.

We develop a data integration method that systematically combines insights from the fields of histopathology and genomics.
Our approach, based on \textit{angle-based joint and individual variation explained} (AJIVE) \cite{feng2018angle}, allows domain experts to explore how information is shared across histopathology and genetic data.
We expect some information to be jointly shared by both data modalities e.g. some tumors are associated with proliferation genes.
Other information may be contained in one modality, but not the other e.g. features of the tumor microenvironment and some genetic subtypes.
By estimating what signals are joint and what signals are modality individual we provide a powerful exploratory analysis framework. 

We apply our approach to the Carolina Breast Cancer Study (CBCS), which provides histologic images and gene expression data for a cohort of breast cancer survivors diagnosed between 2008 and 2013 \citep{troester2017racial}.
The analysis discovers immediately interpretable joint and individual signals. 

\begin{figure}[h]
\centering
\includegraphics[scale=.05]{CBCS3_HE_30030_group_1_image_restained_downsized}
\caption{
A lower resolution view of a \textit{hematoxylin and eosin} (H\&E) stained 1mm core from a breast cancer tissue microarray.
The darker purple color (hematoxylin) stains nuclear material such as DNA, while the pink (eosin) highlights structures such as connective tissue.
% These images are quite large (e.g. $2,500 \times 2,500$ pixels) and complex.
}
\label{fig:he_example}
\end{figure}



Quantitative histopathology means doing statistical analysis of image data. 
We leverage convolutional neural networks (CNNs) for automatic image feature extraction.
CNN features are notoriously difficult to interpret and are not traditionally used for exploratory/inferential analyses.
We develop a multi-scaled approach, \textit{representative patch views} (Section \ref{s:rep_patch_view}), to interpret signals in the histology image data captured by CNN features.
These representative patch views allow experts from different domains (Pathology, Genetics, and Epidemiology) to engage deeply with our analysis. 

The first AJIVE joint component (see Section \ref{ss:results_joint_1}) uncovers tumor grade in the pathology and the Basal-like subtype in the genetics.
This component sorts aggressive tumors with high cellularity into one end of the component and less aggressive, lower cellularity tumors onto the other end of the component.
The association between high grade, Basal-like tumors is well known in the breast cancer literature  \todo{cite} and these tend to be highly aggressive cancers.
The fact this association shows up prominently in the joint information is highly encouraging to domain experts. 

The second joint component (Section \ref{sss:results_joint_2}) identifies previously unknown histologic features of genetically Luminal tumors.
Understanding the histology of Luminal tumors is immediately relevant to clinicians because genetic based testing can be expensive and time consuming.
Currently, little is known about the histology of genetically Luminal tumors \todo{cite}.
Our analysis suggests that retraction artifacts (among other things) can be used by pathologists to identify Luminal B tumors.
These histological features are traditionally ignored by pathologists as artifacts of the tumor processing pipeline. 

The histologic individual AJIVE components (Section \ref{ss:results_image_indiv}) capture features of the tumor microenvironment including \textit{mucinous carcinoma}, high adipose content, and degraded tissue.
These features further validate that we can accurately separate individual information from joint.
The genetic individual AJIVE components (Section \ref{ss:results_genetic_indiv}) contain additional genetic subtype information as well as pick up on well-known technical variation.

%Our analysis presents a number of interesting questions for 
A key challenge in the analysis of complex data is data representation: what do you measure to capture the signal of interest \citep{marron2014overview}?
Automated, data-driven methods for feature extraction such as deep learning have proven to be powerful tools for analyzing complex data in predictive settings \citep{bengio2013representation, couture2018image}.
Leveraging deep learning for exploratory/inferential tasks, where the goal is to learn about patterns in the data, presents new challenges and is an active area of investigation \citep{ash2018joint, adebayo2018sanity,  olah2018building}.


% Inspired by the approach in \cite{couture2018image}, we use an intermediate layer of a pre-trained neural network (see Section \ref{ss:image_pro}) for automatic image feature extraction -- so called \textit{transfer learning} \citep{yosinski2014transferable, sharif2014cnn}.

